Self-supervised Learning of Distance Functions for Goal-Conditioned Reinforcement Learning

Goal-conditioned policies are used in order to break down complex reinforcement learning (RL) problems by using subgoals, which can be defined either in state space or in a latent feature space. This can increase the efficiency of learning by using a curriculum, and also enables simultaneous learning and generalization across goals. A crucial requirement of goal-conditioned policies is to be able to determine whether the goal has been achieved. Having a notion of distance to a goal is thus a crucial component of this approach. However, it is not straightforward to come up with an appropriate distance, and in some tasks, the goal space may not even be known a priori. In this work we learn a distance-to-goal estimate which is computed in terms of the number of actions that would need to be carried out in a self-supervised approach. Our method solves complex tasks without prior domain knowledge in the online setting in three different scenarios in the context of goal-conditioned policies a) the goal space is the same as the state space b) the goal space is given but an appropriate distance is unknown and c) the state space is accessible, but only a subset of the state space represents desired goals, and this subset is known a priori. We also propose a goal-generation mechanism as a secondary contribution.

==> icml2020/sections/appendices/action_space_goal_generation.tex <==
Our algorithm maintains a working set of goals for the policy to train against. The central challenge in designing a curriculum is coming up with a way to ensure that the working set contains as many goals of intermediate difficulty (GOID) as possible. The most straightforward way of generating new GOID goals from old ones is by applying perturbations to the old goals. The downside of this simple approach is that the noise must be carefully tailored to the environment of interest, which places a significant demand for domain knowledge about the nature of the environment's state space. Consider, for instance, that in an environment where the states are represented by images it would be difficult to come up with any kind of noise such that the newly generated states are feasible (i.e. in $S$). Another option is to train a generative neural network to generate new GOID goals, as proposed by GoalGAN \cite{Florensa2018AutomaticGG}; however, this introduces significant additional complexity.

A simple alternative is to employ action space noise. That is, to generate new goals from an old goal, reset the environment to the old goal and take a series of actions using a random policy; take a random subset of the encountered states as the new goals. The states generated in this way are guaranteed to be both feasible and near the agent's current ability. Moreover, applying this approach requires only knowledge of the environment's action space, which is typically required anyway in order to interact with the environment. A similar approach was used in \cite{florensa2017reverse}, but in the context of generating a curriculum of start states growing outward from a fixed goal state.

If implemented without care, action space noise has its own significant drawback: it requires the ability to arbitrarily reset the environment to a state of interest in order to start taking random actions, a strong assumption which is not satisfied for many real-world tasks. Fortunately, we can avoid this requirement as follows. Whenever a goal is successfully achieved during the policy optimization phase, rather than terminating the trajectory immediately, we instead continue for a fixed number of timesteps using the random policy. During the goal selection phase, we can take states generated in this way for GOID goals as new candidate goals. The part of the trajectory generated under the random policy is not used for policy optimization. Note that this combines nicely with the off-policy method for training the distance predictor, as the distance predictor can be trained on these trajectories; this results in a curriculum learning procedure for goal-conditioned policies that requires minimal domain knowledge.

We perform this comparison in both the Maze Ant and Free Ant environments, using $(x, y)$ as the goal space and the Euclidean distance. The results, shown in Fig. \ref{fig:goal_gen_plot}, demonstrate that the performance of our approach is comparable to that of GoalGAN while not requiring the additional complexity introduced by the GAN. The evolution of the working set of goals maintained by our algorithm for Maze Ant is visualized in Fig. \ref{fig:maze_goal_evolution}.

Though our approach requires additional environment interactions, it does not necessarily have a higher sample complexity compared to GoalGAN in the case of indicator reward functions. This is because the goals generated by GoalGAN are not guaranteed to be feasible (unlike our approach); trajectories generated for unfeasible goals will receive 0 reward and will not contribute to learning.

\begin{figure}
  \begin{minipage}{0.48\textwidth}
    \centering
    \subfloat[Maze Ant]{\includegraphics[width=0.5\linewidth]{icml2020/images/goal_generation/goal_gen_maze_l2_xy.png}}
    \subfloat[Free Ant]{\includegraphics[width=0.5\linewidth]{icml2020/images/goal_generation/goal_gen_free_l2_xy.png}}
    \caption{Comparing the proposed goal generation algorithm against GoalGAN. All experiments are averaged over $5$ random seeds.}
    \label{fig:goal_gen_plot}
  \end{minipage}
  \hspace{0.1cm}
    \begin{minipage}{0.48\textwidth}
    \captionsetup[subfigure]{labelformat=empty}
    \centering
    \includegraphics[width=0.98\textwidth, height=2.8cm]{icml2020/images/buffers/buffers.pdf}
    \caption{Evolution of the goals generated by our goal generation approach (top). A sample of goals so-far encountered (bottom),
color-coded according to estimated difficulty: green are easy, blue are GOID and red are hard.}
    \label{fig:maze_goal_evolution}
    \end{minipage}
\end{figure}

==> icml2020/sections/method.tex <==
In order to perform goal-conditioned reinforcement learning, we require a distance function which captures the dynamics of the environment. Roughly, we would like a distance function which is small if and only if the goal can be reached from the state in a small number of steps, and, importantly, ignores incindental details such as how similar the two states are on the surface, e.g. their L2 distance.

\subsection{Average Commute Time}
We will start by considering a Markov Decision Process with a fixed policy $\pi$, forming a Markov chain.
The average first passage time from state $i$ to $j$ is defined as the expected number of steps to reach $j$ for the first time after starting from $i$. Using the notation in \cite{Fouss:2005:NWC:1092358.1092536}, we write the average first passage time $m(j|i)$ recursively as 
\begin{equation*}
    m(j|i) = \begin{cases}
                1 + \sum_{k \in S} P(k|i) m(k|i) & i \neq j \\
                0 & otherwise
             \end{cases}
\end{equation*}
A related quantity, the average commute time $n(i, j)$ is defined as $n(i,j)=m(i|j) + m(j|i)$. Average commute time is a distance metric as noted in \cite{Fouss:2005:NWC:1092358.1092536}. Let $X(t)$ be the random variable that denotes the state at time $t$. Then $m(i|j)$ can be alternatively expressed as $\mathbf{E}[T_{ij}]$, where $T_{ij}=min\{t \geq 0: X(t)=j\}$ given $X(0)=i$.

\subsection{Commute Time Embeddings}
\cite{Fouss:2005:NWC:1092358.1092536} proposed to define a measure of similarity of nodes in weighted undirected graphs using Markov chain based distances based on random walk on graphs and show the existence of an Euclidean embedding space where the distance between embeddings of nodes $i$ and $j$ correspond to the square root of the average commute time between them, $\sqrt{n(i,j)}$. 

They used this embedding space to obtain a low dimensional representation of the graph. Further, they show the relationship between such an Euclidean space and the pseudo-inverse of the Laplacian $L^{\dagger}$. The representation of node $i$ is the $i^{th}$ row of $Q\Lambda^{\frac{1}{2}}$ where the columns of $Q$ are the eigenvectors of $L^{\dagger}$ and $\Lambda$ is a diagonal matrix of the corresponding eigenvalues. This is also the solution given by cMDS when $D^2(X)_{ij}=n(i,j)$ or when $B_{ij}=L^\dagger_{ij}$. We provide further discussion in \ref{sec:ectd}. However, neither the matrix of pairwise commute times nor $L^{\dagger}$ are available in RL and hence cMDS cannot be applied. \textbf{Therefore, we estimate the pairwise commute times based on the trajectories and use metric MDS to find the embedding space that preserves commute time distances. Further discussion is presented in \ref{sec:approx_with_mmds}.}

cMDS can be used to recover the embedding in the case of a finite state-space.

\subsection{Approximate, Online MMDS}
We propose to learn a task specific distance function where the distance between states $s_1$ and $s_2$ is defined as the \textbf{half of del(\textit{the  expected number of actions under a policy $\pi$ required to reach $s_2$ from $s_1$ \textbf{for the first time} and return to $s_1$}) commute-time} which we call the \textit{action distance}.  Defining the distance in terms of reachability of the states captures the environment dynamics as experienced by the agent under the policy $\pi$. In order to learn a distance estimator we propose to learn an embedding such that the distance between the embeddings of a pair of states is equal to the action distance between the states.

\textbf{(todo: update the notations to reflect first passage time)}Formally, let $s_i, s_j \in \mathcal{S}$, and define the action distance $d^\pi(s_i, s_j)$ as:
\begin{align}
    d^{\pi}(s_i, s_j) = E_{\tau \sim \pi, m \sim \overline{t}(s_i, \tau), n \sim \overline{t}(s_j, \tau)} \left[|m - n |\right]
\end{align}
where $\overline{t}(s, \tau)$ is a uniform distribution over all temporal indices of $s$ in $\tau$ and the expectation is taken over trajectories $\tau$ sampled from $\pi$ such that $s_i$ and $s_j$ both occur in $\tau$. If $\pi$ is a goal-conditioned policy we also average over goals $g$ provided to $\pi$.
 %and $k \in \mathbb{N}$ be an integer. Two points $(s_i,s_j)$ are said to be $k$-close under $\pi$ if $s_i$ is reachable from $s_j$ within $k$ actions under the policy $\pi$ and vice-versa. We denote the distance-action between $(s_i,s_j)$ as $d^{\pi}(s_i,s_j)$.
%($d^{\pi}_{ij}$ in short).

In general, $d^\pi(s_i, s_j)$ is difficult to compute; this is problematic, since this distance is intended to be used for detecting when goals have been achieved and will be called frequently. Therefore, we propose to train a neural network to estimate it. Specifically, we learn an embedding function $e_\theta$ of the state space, parameterized by vector $\theta$, such that the $p$-norm between a pair of embedding is close to the action distance between the corresponding states. The objective function used to train $e_\theta$ is:
\begin{equation}
\label{eq:1}
    \theta^* = \argmin_\theta (||e_\theta(s_i) - e_\theta(s_j)||_p^q - d^{\pi}(s_i, s_j))^2
\end{equation}
% Learning an embedding with Equation \eqref{eq:1} as the objective function
% %property (\ref{eq:1})
% is an instance of metric multidimensional scaling. \textbf{We discuss the relationship of our approach to MDS and the connection to the graph Laplacian in the next section. As a result of the discussion, we show that our approach, under some assumptions, is an approximation of a theoretically optimal quantity and why a space where the euclidean distance between states corresponding to action distance exists.}

\subsection{On-policy vs Off-policy Learning}
When used as part of a goal-conditioned policies, the distance predictor can be trained using the trajectories collected by the behavior policy during the policy-learning phase. We call this case the \textit{on-policy} distance predictor. We emphasize that the on-policy nature of this distance predictor is independent of whether the policies or value functions are on-policy.
% In this case the embedding function is specific to the policy conditioned on goal $g$ and similarly $d^{\pi}$ is action distance with respect to the policy conditioned on $g$. 
While such an on-policy distance possesses desirable properties, such as a simple training scheme, it also has drawbacks. Both the behavior policy and goal distribution will change over time and thus the distance function will be non-stationary.
% This non-stationarity will be problematic if the distance predictor is to be used to make decisions such as whether or not to add goals to a goals replay buffer. For instance, goals that were farther in number of actions under the initial policy can become closer under a trained policy.
% This results in computational overhead in maintaining the components like the goals buffer that are dependent on the distance predictor.
This can create a number of issues, the most important of which is difficulty in setting the threshold $\epsilon$. Recall that in our setting, the goal is considered to be achieved and the episode terminated once $d^\pi(s, g) < \epsilon$ where $\epsilon$ is a threshold hyperparameter.
This thresholding creates an $\epsilon$-sphere around the goal, with the episode terminating whenever the agent enters this sphere. The interaction between the $\epsilon$-sphere and the non-stationarity of the on-policy distance function cause a subtle issue that we dub the \textit{expanding $\epsilon$-sphere} phenomenon, discussed in detail in Section \ref{sec:expanding_sphere}.
% Moreover, in goal-conditioned policies, a collection of policies is learned simultaneously, one for each goal. Hence, the distance between two states $s_1$ and $s_$ will also depend on the goal $g$. 

An alternative approach to learning the distance function from the trajectories generated by the behavior policy is to apply a random policy for a fixed number of timesteps at the end of each episode. The states visited under the random policy are then used to train the distance function. Specifically, we take the trajectories generated by the random policy for obtaining new goals, and re-use them to train the distance function. Since the random policy is independent of the behavior policy, we describe the learned distance function as \textit{off-policy} in this case. The stationarity of the random policy helps in overcoming the expanding $\epsilon$-sphere phenomenon of the on-policy distance predictor.
